UniPoll: A Unified Social Media Poll Generation Framework via Multi-Objective Optimization

Social media platforms are vital for expressing opinions and understanding public sentiment, yet many analytical tools overlook passive users who mainly consume content without engaging actively. To address this, we introduce UniPoll, an advanced framework designed to automatically generate polls from social media posts using sophisticated natural language generation (NLG) techniques. Unlike traditional methods that struggle with social media's informal and context-sensitive nature, UniPoll leverages enriched contexts from user comments and employs multi-objective optimization to enhance poll relevance and engagement. To tackle the inherently noisy nature of social media data, UniPoll incorporates Retrieval-Augmented Generation (RAG) and synthetic data generation, ensuring robust performance across real-world scenarios. The framework surpasses existing models, including T5, ChatGLM3, and GPT-3.5, in generating coherent and contextually appropriate question-answer pairs. Evaluated on the Chinese WeiboPolls dataset and the newly introduced English RedditPolls dataset, UniPoll demonstrates superior cross-lingual and cross-platform capabilities, making it a potent tool to boost user engagement and create a more inclusive environment for interaction.

==> others/biography.tex <==



\vspace{-33pt}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/biography/YixiaLi.jpeg}}]{Yixia Li}
received the M.Sc. degree from The Hong Kong Polytechnic University (PolyU), Kowloon, Hong Kong, in 2023.
He was a Research Assistant from February 2022 to January 2023 with the Department of Computing of The Hong Kong Polytechnic University. He is currently a PhD student at the Department of Statistics and Data Science of the Southern University of Science and Technology. 
His research interests include data synthesis, controllable text generation and multi-modal.
\end{IEEEbiography}

\vspace{-33pt}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/biography/RongXiang.jpeg}}]{Rong Xiang} is a postdoctoral fellow working in the Department of Computing, The Hong Kong Polytechnic University (PolyU) since 2022. He obtained his Ph.D. degree from the same department in 2022. Before that, he obtained two M.Sc. degrees in artificial intelligence from the University of Edinburgh, United Kingdom in 2015; and an M.Sc. degree in information engineering from Zhejiang University, Hangzhou, China in 2013. Between 2015 and 2017, he worked as a software engineer at Advanced Micro Devices Inc. in Shanghai. Rong has broad research interests in large language models, multi-modal machine learning, and natural language processing. He is particularly dedicated to applying advanced AI solutions across various industries, with a strong focus on contributing to AI for Good initiatives.

\end{IEEEbiography}

\vspace{-33pt}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/biography/YanlinSong.jpeg}}]{Yanlin Song} received the M.Sc. degree in data science and analytics from The Hong Kong Polytechnic University in 2024. She is currently working towards an PhD degree with the computer science and technology in Wuhan University. Her research interests include LLM and knowledge graph.
\end{IEEEbiography}

\vspace{-33pt}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/biography/JingLi.jpeg}}]{Jing Li} is an Assistant Professor of the Department of Computing (COMP), Hong Kong Polytechnic University (PolyU) since 2019. She established and currently leads the PolyU Embodied Artificial Intelligence Lab under PolyU-COMP and is a member of the PolyU Research Centre on Data Sciences \& Artificial Intelligence (RC-DSAI). Before joining PolyU, she was a senior researcher at NLP Center, Tencent AI Lab from 2017 to 2019. Jing obtained her PhD degree from the Department of Systems Engineering and Engineering Management, Chinese University of Hong Kong in 2017. Before that, she received her B.S. degree from the Department of Machine Intelligence, Peking University in 2013.
\end{IEEEbiography}

==> tables/english_weibopolls.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}
\begin{table}
    \centering
    \caption{\hl{Poll generation results on English \textit{WeiboPolls} through back-translation.}}
    \label{tab:english_weibopolls}
    \resizebox{1\columnwidth}{!}
    {
    \begin{tabular}{|l|rrrr|}
    \hline
    \multirow{2}{*}{\textbf{Model}} & \multicolumn{4}{c|}{\textbf{Poll Generation}}   \\
               & \multicolumn{1}{c}{\textbf{ROUGE-1}} & \multicolumn{1}{c}{\textbf{ROUGE-L}} & \multicolumn{1}{c}{\textbf{BLEU-1}} & \multicolumn{1}{c|}{\textbf{BLEU-3}} \\ \hline
    {\ul \textbf{Current SOTA}}     &                 &                 &                &                 \\
    GPT-2 & 26.17         & 17.18          & 18.70         & 10.85          \\
    Bart-base & 32.58         & 24.57          & 19.09         & 14.25          \\
    T5-Pegasus & 53.46         & 44.18          & 42.85         & 32.18          \\ \hline
    {\ul \textbf{LLM}}     &                 &                 &                &                 \\
    GPT-4   & 38.10         & 29.08          & 29.13         & 13.04          \\ \hline
    {\ul \textbf{Our Model}}        &                 &                 &                &                 \\
    UniPoll    & \textbf{53.57}  & \textbf{44.87}  & \textbf{43.63} & \textbf{32.79}  \\ \hline
    \end{tabular}
    }
\end{table}
